SimSAM: Zero-shot Medical Image Segmentation via Simulated Interaction

The recently released Segment Anything Model (SAM) has shown powerful zero-shot segmentation capabilities through a semi-automatic annotation setup in which the user can provide a prompt in the form of clicks or bounding boxes. There is growing interest around applying this to medical imaging, where the cost of obtaining expert annotations is high, privacy restrictions may limit sharing of patient data, and model generalisation is often poor. However, there are large amounts of inherent uncertainty in medical images, due to unclear object boundaries, low-contrast media, and differences in expert labelling style. Currently, SAM is known to struggle in a zero-shot setting to adequately annotate the contours of the structure of interest in medical images, where the uncertainty is often greatest, thus requiring significant manual correction. To mitigate this, we introduce \textbf{Sim}ulated Interaction for \textbf{S}egment \textbf{A}nything \textbf{M}odel (\textsc{\textbf{SimSAM}}), an approach that leverages simulated user interaction to generate an arbitrary number of candidate masks, and uses a novel aggregation approach to output the most compatible mask. Crucially, our method can be used during inference directly on top of SAM, without any additional training requirement. Quantitatively, we evaluate our method across three publicly available medical imaging datasets, and find that our approach leads to up to a 15.5\% improvement in contour segmentation accuracy compared to zero-shot SAM. Our code is available at \url{https://github.com/BenjaminTowle/SimSAM}.

==> src/2_related_work.tex <==
For related work, we first discuss the applications of previous work to the Segment Anything Model; next, we consider work on interactive Medical Image Segmentation which is a motivational paradigm for our method; then, we consider approaches to uncertainty estimation in medical imaging; finally, we consider previous approaches to creating stochastic segmentation models in medical imaging.

\paragraph{Medical Imaging in SAM}
Since the release of the Segment Anything Model, there has been a groundswell of works seeking to evaluate the capabilities of SAM in medical imaging. One line of work evaluates the effectiveness of the available prompting strategies for SAM, e.g. clicks and bounding-boxes. Among these, \cite{medsam2} find bounding boxes to be the most effective form of interaction. This is also corroborated by \cite{medsam-zs} who find the bounding box approach outperforms even much larger numbers of clicks.  Other research compares SAM directly to existing approaches: \cite{He2023AccuracyOS} find SAM underperforms other popular supervised approaches such as the U-Net \cite{Ronneberger2015UNetCN}; similar results are observed by \cite{Ji2023SegmentAI}, who find that SAM requires some level of human prompting to perform meaningfully out-of-the-box. Another line of research attempts to finetune SAM on downstream medical imaging datasets. \cite{medsam2} introduce MedSAM, a version of SAM finetuned on numerous medical datasets, although performance still lags behind bespoke models. \cite{Wu2023MedicalSA} introduce a parameter efficient fine-tuning adapter to SAM, enabling SAM to learn from medical images without catastrophic forgetting.   

\paragraph{Interactive Medical Image Segmentation}
Due to the challenges of obtaining accurate, automatically-segmented medical images, many works consider the interactive setup, in which the expertise of a human annotator can be leveraged to refine the model predictions \cite{Zhao2013AnOO, Masood2015ASO}. There is a rich range of interaction types have been explored such as clicks \cite{Sakinis2019InteractiveSO ,Wang2017DeepIGeoSAD}, bounding boxes \cite{Rajchl2016DeepCutOS ,Wang2017InteractiveMI}, or scribbles \cite{Wang2017DeepIGeoSAD}. For pre-trained models, recent work finds bounding boxes to be the most effective form of interaction \cite{medsam}. Where previous work uses interaction for systems that will be directly interacted with by real users, we repurpose the framework of user interaction for simulation and use the uncertainty around user behaviour to generate multiple plausible hypotheses.  The closest to our work is arguably \cite{Liu2022PseudoClickII}, who learn to predict user clicks and use user simulation to iteratively improve the model's predictions. However, unlike our method, their method requires additional training of a separate model to predict user clicks, rather than being extracting from the model's existing knowledge.

\paragraph{Uncertainty Estimation}
Uncertainty estimation (or quantification) is a key part of medical imaging models, as it allows the model to flag cases to the user where its predictions may be inaccurate and therefore require additional scrutiny \cite{Zou2023ARO}. There are broadly four classes of approaches that have been proposed: (i) deterministic methods explicitly produce an uncertainty score (e.g. outputting an expected IoU score \cite{sam}); (ii) Bayesian neural networks represent model parameters as random variables \cite{maddox2019simple, Awate2019EstimatingUI}, enabling multiple predictions to be sampled for each input. To compensate for the slowness of training this method, Monte-Carlo dropout methods have also been proposed as a faster extension \cite{Yu2019UncertaintyawareSM}, which provide an approximation of Bayesian methods through applying random dropout layers; (iii) ensemble-based methods train multiple models on the same task, and then use model disagreement as a proxy for uncertainty \cite{Cao2020UncertaintyAT}; (iv) test-time augmentation produce different outputs by applying various permutations and distortions to the inputs \cite{Wang2018AleatoricUE}. We note that most of these approaches require specific training regimes, rather than being usable in a zero-shot setting. Most relevant to our work are the deterministic methods, as they form the baseline approach used by the SAM pre-trained model, via its regression-based IoU prediction heads.

\paragraph{Stochastic Medical Imaging}
Adjacent to the work on uncertainty estimation, other works have sought to explicitly represent uncertainty in medical images through designing architectures that enable segmentation masks to be sampled, in contrast to deterministically mapping the input to a single dense pixel-wise output. \cite{Kohl2018APU} introduce a probabilistic variant of the popular U-Net through the use of latent variables. However, as this often still led to relatively deterministic outputs (i.e. mode collapse), \cite{Baumgartner2019PHiSegCU} and \cite{Kohl2019AHP} both introduce hierarchical latent variables to increase the model's expressive power. 
\cite{Monteiro2020StochasticSN} learn to represent the output logits as a probability distribution; finally, \cite{Rahman2023AmbiguousMI} use a diffusion model to generate annotations. However, none of these approaches can be directly applied in the zero-shot setting, as they all require specific training. By contrast, in this study, SimSAM can be built directly on top of SAM with no additional training required. 

%\paragraph{Multiple Hypothesis Prediction}
%The task of Multiple Hypothesis Prediction (MHP) is concerned with explicitly representing uncertainty through the production of multiple outputs, in contrast to the standard machine learning paradigm of predicting only a single output \cite{Rupprecht2016LearningIA, Firman2018DiverseNetWO}. MHP occupies a growing body of research across various machine learning tasks ranging from dialogue reply suggestion \cite{Deb2019DiversifyingRS, Towle2023ModelBasedSF}, to future prediction \cite{Rupprecht2016LearningIA, Berlati2020AmbiguityIS, Wang2023DearNetLD}, 3D shape generation \cite{Firman2018DiverseNetWO}, and model-based reinforcement learning \cite{Seo2020TrajectorywiseMC, Yuan2022EUCLIDTE} and image segmentation \cite{GuzmnRivera2012MultipleCL, GuzmnRivera2014EfficientlyED, Lee2016StochasticMC, Tian2019VersatileMC, sam}. In computer vision, early work in MHP introduced the concept of Multiple Choice Learning (MCL), which, partially inspired by ensemble-based methods, optimised a set of models by iteratively assigning samples to the most accurate (i.e. `oracle') model, followed by re-training with those assignments, in a process analogous to the Expectation Maximisation (EM) algorithm \cite{GuzmnRivera2012MultipleCL}. This was expanded upon with DivMCL which used a diversity-based multitask loss to enforce greater diversity in the model predictions \cite{GuzmnRivera2014EfficientlyED}. The MCL framework was later applied to deep neural networks \cite{Lee2016StochasticMC}, where the EM process was replaced by only backpropagating through the most accurate model for each sample. This enabled the entire architecture to be trained in a single run, making the techniques feasible for the longer training times associated with deep learning. Additional work has also been done to deal with overconfidence in prediction heads \cite{Lee2017ConfidentMC, Tian2019VersatileMC}, while other work \cite{Firman2018DiverseNetWO} generalised the MCL framework to the scenario with multiple labels. Most recently, the SAM pre-trained model was released \cite{sam}, which directly incorporates MCL as part of its training strategy. In medical imaging, several methods for producing multiple outputs have been proposed, such as probabilistic variants of the popular U-Net \cite{Kohl2018APU}, sequential latent variables \cite{Baumgartner2019PHiSegCU}, learning the covariance between output logits \cite{Monteiro2020StochasticSN}, or training diffusion models \cite{Rahman2023AmbiguousMI}. However, all these approaches require training on target datasets containing one or more pixel-level annotations per image. In other words, they can only be used as a downstream application, rather than as a tool for generating multiple annotations in novel domains. Contrastingly, in this study, we consider the question of \textit{how can multiple accurate and diverse annotations be generated without domain-specific training}. 

%\paragraph{Intrinsic Motivation}
%Due to the sparsity of rewards in many reinforcement learning problems, several approaches consider intrinsic motivation, which allows the model to optimise a (usually dense) calculable internal reward function. There are broadly two instantiations of motivating an intrinsic motivation agent \cite{Pathak2017CuriosityDrivenEB}: (i) novelty-based methods, which encourage the model to obtain novel states \cite{Bellemare2016UnifyingCE, Stadie2015IncentivizingEI}, or (ii) learning-based methods that reward the model for improving its predictive model of the world \cite{Houthooft2016VIMEVI, Schmidhuber2010FormalTO}. Between these, our approach of rewarding diverse actions is more closely related to (i). A key challenge is how to define and measure the novelty of a particular state, particularly when the state-space is large, as is the case in image segmentation.  Several previous works use learned density models to predict pseudo-counts \cite{Bellemare2016UnifyingCE, Ostrovski2017CountBasedEW} \brevision{-- this enables estimating the novelty of a particular state, even where the state space is sufficiently large that each exact state is unlikely to be revisited.} Unlike these methods however, which involve learning a parametric agent during training, we instead focus on solving this problem as an online planning problem. Several previous works apply IM to the model-based RL paradigm \cite{Sekar2020PlanningTE, Lowrey2018PlanOL}. To the best of our knowledge, this work is the first to apply intrinsic motivation to either the image segmentation or multiple hypothesis prediction tasks.
%Unlike these however, our method has the advantage of not requiring a learned simulator, as the environment dynamics are already known -- i.e. our state consists of the currently selected masks,  

